Stepwise Alignment for Constrained Language Model Policy Optimization

Safety and trustworthiness are indispensable requirements for real-world applications of AI systems using large language models (LLMs). This paper formulates human value alignment as an optimization problem of the language model policy to maximize reward under a safety constraint, and then proposes an algorithm, Stepwise Alignment for Constrained Policy Optimization (SACPO). One key idea behind SACPO, supported by theory, is that the optimal policy incorporating reward and safety can be directly obtained from a reward-aligned policy. Building on this key idea, SACPO aligns LLMs step-wise with each metric while leveraging simple yet powerful alignment algorithms such as direct preference optimization (DPO). SACPO offers several advantages, including simplicity, stability, computational efficiency, and flexibility of algorithms and datasets. Under mild assumptions, our theoretical analysis provides the upper bounds on optimality and safety constraint violation. Our experimental results show that SACPO can fine-tune Alpaca-7B better than the state-of-the-art method in terms of both helpfulness and harmlessness.

==> body/15_pessimism.tex <==
\section{Incorporating Pessimism}

\red{Under construction below}

\textit{Pessimism} is a well-known principle in offline RL settings where an agent optimizes its policy using a fixed amount of dataset that has been collected previously~\cite{jin2021pessimism,xie2021bellman}.
In our problem settings, the upper bounds in Theorems~\ref{theorem:optimality} and \ref{theorem:safety} can also be improved by incorporating pessimism.
Specifically, let us consider the case where the policy is optimized with respect to the pessimistic estimates of the reward and safety functions; that is, for any positive scalar $c \in [0, \Lambda]$,
%
\begin{align*}
    \bar{\pi}(\ymidx) \coloneqq \frac{1}{\Z{\bar{h}}{\piref}} \piref \exp\left(\frac{1}{\beta} \bar{h} \xy \right), \quad \text{with} \quad \bar{h} \xyc \coloneqq \widehat{h} \xy - \widehat{\Gamma}_\calD(x, y, c).
\end{align*}

We now present a lemma similar to Lemma~\ref{lem:decom}.
%
\begin{lemma}
\label{lem:decom_pessimism}
    For any function $f: \calX \times \calY \rightarrow \mbR$ and policy $\pi \in \Pi$, define a function such that
    %
    \begin{equation*}
        J_f(\pi) \coloneqq \mbE_\rho \Big[\mbE_{\pi}[f \xy] - \beta\KL{\pi(\ymidx)}{\piref(\ymidx)} \Big].
    \end{equation*}
    %
    Then, the following equation holds:
    %
    \begin{alignat}{2}
        \nonumber
        &J_{\eta_c^\star}(\piopt) - J_{\eta_c^\star}(\pihat) \\
        &\qquad = \mbE_\rho \left[{\mbE_{\piopt}[\eta_c^\star \xy - h^\star\xy]}
        + {\mbE_{\pihat}[\bar{h} \xyc - \eta_c^\star \xy]}
        + \beta \log \frac{Z_{h^\star}(x; \piref)}{Z_{\bar{h}}(x; \piref)}\right].
        \label{eq:decom_pessimism}
    \end{alignat}
\end{lemma}

\begin{proof}
    This lemma directly follows from Lemma~\ref{lem:decom} with a minor change from $\widehat{h}$ to $\bar{h}$.
\end{proof}

We now derive the upper bound of each term in \eqref{eq:decom_pessimism}.
Since the first term is identical to the one in Lemma~\ref{lemma:hopt_hhat_1}, we will discuss the second and third terms.
%
\begin{lemma}
    \label{lemma:pessimism_negative}
    Set $\widehat{\lambda}$ such that $\widehat{\lambda} \ge c$.
    Then, the following inequality holds:
    %
    \begin{equation}
        \mbE_\rho \Bigl[\mbE_{\pihat}[\,\bar{h} \xyc - \eta_c^\star \xy] \Bigr] \le 0.
    \end{equation}
\end{lemma}
%
\begin{proof}
    By definition,
    %
    \begin{align*}
        \bar{h} \xyc - \eta_c^\star \xy
        =
        \widehat{h} \xy - \widehat{\Gamma}_\calD(x, y, c) - \eta_c^\star \xy.
    \end{align*}
    
    By Lemma~\ref{lem:uncertainty_h}, we have
    %
    \begin{align*}
        \widehat{h} \xy - \widehat{\Gamma}_\calD(x, y, c) - \eta_c^\star \xy \le 0.
    \end{align*}
    %
    Therefore, we have the desired lemma.
\end{proof}

\begin{lemma}
    \label{lemma:upper_bound_z_pessimism}
    For any $x \in \calX$, the following inequality holds:
    %
    \begin{align*}
        \frac{ \Z{h^\star}{\piref}}{\Z{\bar{h}}{\piref}}
        \le \mbE_{\piopt} \left[\exp\left(\frac{1}{\beta} \left(\widehat{\Gamma}_\calD \xyc + \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right)\right) \right].
    \end{align*}
\end{lemma}

\begin{proof}
    For any $x \in \calX$, the following chain of equalities holds:
    %
    \begin{align*}
        \frac{ \Z{h^\star}{\piref}}{\Z{\bar{h}}{\piref}}
        &= \frac{ \Z{h^\star}{\piref}}{ \sum_{y} \piref(\ymidx) \exp\left(\frac{1}{\beta} \bar{h}\xyc \right)}
        \\ 
        &= \frac{ \Z{h^\star}{\piref}}{ \sum_{y} \piref(\ymidx) \exp\left(\frac{1}{\beta} h^\star\xy\right) \exp\left(\frac{1}{\beta} \left(\bar{h}\xyc - h^\star \xy\right)\right)}
        \\
        &\le \frac{ \Z{h^\star}{\piref}}{ \sum_{y} \piref(\ymidx) \exp\left(\frac{1}{\beta} h^\star\xy\right) \exp\left(-\frac{1}{\beta} \left|\, \bar{h}\xyc - h^\star \xy \,\right|\right)}.
    \end{align*}
    %
    By definition of $\bar{h}$, we have
    %
    \begin{align*}
        \left|\, \bar{h}\xyc - h^\star \xy \,\right| 
        & = \left|\, \widehat{h}\xy - \widehat{\Gamma}_\calD \xyc - h^\star \xy \,\right| \\
        & \le \left|\, \widehat{h}\xy - h^\star \xy \,\right| + \left|\, \widehat{\Gamma}_\calD \xyc \,\right| \\
        & \le \widehat{\Gamma}_\calD (x, y, \lambdaopt) +  \widehat{\Gamma}_\calD \xyc.
    \end{align*}
    %
    \begin{align*}
        \frac{ \Z{h^\star}{\piref}}{\Z{\bar{h}}{\piref}}
        &\le \frac{ \Z{h^\star}{\piref}}{ \sum_{y} \piref(\ymidx) \exp\left(\frac{1}{\beta} h^\star\xy\right) \exp\left(-\frac{1}{\beta} \widehat{\Gamma}_\calD \xyc \right) \exp\left(-\frac{1}{\beta} \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right)}
        \\
        &= \frac{1}{ \mbE_{\piopt} \left[\exp\left(-\frac{1}{\beta} \widehat{\Gamma}_\calD \xyc \right) \exp\left(-\frac{1}{\beta} \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right) \right]}
        \\
        &\le  \mbE_{\piopt} \left[\exp\left(\frac{1}{\beta} \left(\widehat{\Gamma}_\calD \xyc + \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right)\right) \right].
    \end{align*}
    %
    In the above transformation, we used the definition of $\Z{h^\star}{\piref}$; that is,
    %
    \begin{equation*}
        \Z{h^\star}{\piref} \coloneqq \sum_{y} \piref(\ymidx) \exp\left(\frac{1}{\beta} h^\star\xy\right). 
    \end{equation*}
    %
    Therefore, we have the desired lemma.
\end{proof}

\begin{lemma}
    \label{lemma:J_eta_c_pessimism}
    The following inequality holds:
    %
    \begin{alignat*}{2}
    J_{\eta^\star_c}(\piopt) - J_{\eta^\star_c}(\bar{\pi})
    \le
    (c - \lambdaopt) b + 
    \beta \log \left(\mbE_{\rho,\piopt} \left[\exp\left(\frac{1}{\beta} \left(\widehat{\Gamma}_\calD \xyc + \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right)\right) \right] \right).
    \end{alignat*}
\end{lemma}
%
\begin{proof}
    In Lemma~\ref{lem:decom_pessimism}, set $f \xy = \eta^\star_c \xy$ for all $\xy \in \calX \times \calY$ and then combining it with Lemmas \ref{lemma:hopt_hhat_1}, \ref{lemma:pessimism_negative}, and \ref{lemma:upper_bound_z_pessimism},
    
    \begin{alignat*}{2}
        J_{\eta^\star_c}(\piopt)& - J_{\eta^\star_c}(\pihat) \\
        =
        &\  
        \mbE_\rho \left[{\mbE_{\piopt}[\eta^\star_c \xy - h^\star\xy]}
        + {\mbE_{\pihat}[\widehat{h} \xy - \eta^\star_c \xy]}
        + \beta \log \frac{Z_{h^\star}(x; \piref)}{Z_{\widehat{h}}(x; \piref)}\right]\\
        \le 
        &\ 
        (c - \lambdaopt) b
        + \beta \log \left(\mbE_{\rho,\piopt} \left[\exp\left(\frac{1}{\beta} \left(\widehat{\Gamma}_\calD \xyc + \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right)\right) \right] \right).
    \end{alignat*}
\end{proof}

\begin{theorem}
    \label{theorem:optimality_pessimism}
    Let $\bar{\pi}$ denote the optimal policy induced by $\bar{h}$.
    Then, the following inequality holds:
    %
    \begin{alignat*}{2}
        R(\piopt, \beta) - R(\bar{\pi}, \beta)
        \le - \lambdaopt b + \beta \log \left(\mbE_{\rho,\piopt} \left[\exp\left(\frac{1}{\beta} \left(\widehat{\Gamma}_\calD (x, y, 0) + \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right)\right) \right] \right).
    \end{alignat*}
\end{theorem}

\begin{proof}
    Set $c = 0$ in Lemma~\ref{lemma:J_eta_c_pessimism}.
    Then we immediately obtain the desired theorem.
\end{proof}

\begin{theorem}[Safety constraint violation]
    \label{theorem:safety_pessimism}
    Suppose that the \algoshort~algorithm identifies that $\pihat$ satisfies the safety constraint based on its evaluation; that is, $\mbE_{\rho, \pihat}[\, \widehat{g} \xy\,] \ge b$.
    Then, we have
    %
    \begin{alignat*}{2}
        [\, b - G(\pihat)\,]_+
        \le \alpha \, \mbE_{\rho, \piopt}\left[\, \calU_{\calD_g} \xy \exp\left(\frac{2}{\beta} \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right) \right].
    \end{alignat*}
\end{theorem}

\begin{proof}
    When the safety constraint is satisfied (i.e., $G(\pi) \ge b$), Theorem~\ref{theorem:safety} is trivially true.
    Therefore, we consider the case of $G(\pi) \le b$.
    
    By definition of $G(\cdot)$, we have the following chain of inequalities:
    %
    \begin{alignat*}{2}
        b - G(\bar{\pi}) 
        = &\ b - \mbE_{\rho, \bar{\pi}}[\, g^\star \xy\,] \\
        = &\ b - \mbE_{\rho, \bar{\pi}}[\, \widehat{g} \xy\,] + \mbE_{\rho, \bar{\pi}}[\, \widehat{g} \xy\,] -\mbE_{\rho, \bar{\pi}}[\, g^\star \xy\,]. 
    \end{alignat*}

Here, we suppose that the \algoshort~algorithm identifies that $\bar{\pi}$ satisfies the safety constraint based on its evaluation; that is,
%
\begin{equation}
    \mbE_{\rho, \bar{\pi}}[\, \widehat{g} \xy\,] \ge b.
\end{equation}

Therefore, we have the following chain of inequalities:
%
\begin{alignat*}{2}
    b - G(\bar{\pi}) 
    \le &\ \mbE_{\rho, \bar{\pi}}[\, \widehat{g} \xy\,] -\mbE_{\rho, \bar{\pi}}[\, g^\star \xy\,] \\
    = &\ \mbE_{\rho, \bar{\pi}}[\, \widehat{g} \xy - g^\star \xy\,] \\
    = &\ \mbE_{\rho, \bar{\pi}}\left[\, \frac{\bar{\pi}(\ymidx)}{\piopt(\ymidx)} \bigl(\widehat{g} \xy - g^\star \xy \bigr) \,\right] \\
    = &\ \mbE_{\rho, \bar{\pi}}\left[\, \frac{\bar{\pi}(\ymidx)}{\piopt(\ymidx)} \cdot \alpha \, \calU_{\calD_g} \xy \,\right].
\end{alignat*}
%
By definition of $\bar{\pi}$, the following chain of equation holds:
%
\begin{align*}
    \frac{\bar{\pi}(\ymidx)}{\piopt(\ymidx)}
    & = \frac{\Z{h^\star}{\piref}}{\Z{\bar{h}}{\piref}} \exp \left(\frac{1}{\beta} \left(\bar{h} \xyc - h^\star \xy \right)\right) \\
    & \le \mbE_{\piopt} \left[\exp\left(\frac{1}{\beta} \left(\widehat{\Gamma}_\calD \xyc + \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right)\right) \right].
\end{align*}

\begin{alignat*}{2}
    b - G(\bar{\pi}) 
    \le &\ \mbE_{\rho, \bar{\pi}}[\, \widehat{g} \xy\,] -\mbE_{\rho, \bar{\pi}}[\, g^\star \xy\,] \\
    = &\ \mbE_{\rho, \bar{\pi}}[\, \widehat{g} \xy - g^\star \xy\,] \\
    = &\ \mbE_{\rho, \bar{\pi}}\left[\, \frac{\bar{\pi}(\ymidx)}{\piopt(\ymidx)} \bigl(\widehat{g} \xy - g^\star \xy \bigr) \,\right] \\
    = &\ \mbE_{\rho, \bar{\pi}}\left[\, \frac{\bar{\pi}(\ymidx)}{\piopt(\ymidx)} \cdot \alpha \, \calU_{\calD_g} \xy \,\right] \\
    \le &\ \mbE_{\rho, \piopt}\left[\, \exp\left(\frac{2}{\beta} \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right) \cdot \alpha \, \calU_{\calD_g} \xy \right] \\
    = &\ \alpha \, \mbE_{\rho, \piopt}\left[\, \calU_{\calD_g} \xy \exp\left(\frac{2}{\beta} \widehat{\Gamma}_\calD (x, y, \lambdaopt) \right) \right].
\end{alignat*}

The transformation from the third to fourth lines follows from Lemma~\ref{lemma:uncertainty} and Lemma~\ref{lemma:ipw}.

Therefore, we obtained the desired theorem.
\end{proof}
